Code-switched inspired losses for generic spoken dialog representations

Spoken dialog systems need to be able to handle both multiple languages and multilinguality inside a conversation (\textit{e.g} in case of code-switching). In this work, we introduce new pretraining losses tailored to learn multilingual spoken dialog representations. The goal of these losses is to expose the model to code-switched language. To scale up training, we automatically build a pretraining corpus composed of multilingual conversations in five different languages (French, Italian, English, German and Spanish) from \texttt{OpenSubtitles}, a huge multilingual corpus composed of 24.3G tokens. We test the generic representations on \texttt{MIAM}, a new benchmark composed of five dialog act corpora on the same aforementioned languages as well as on two novel multilingual downstream tasks (\textit{i.e} multilingual mask utterance retrieval and multilingual inconsistency identification). Our experiments show that our new code switched-inspired losses achieve a better performance in both monolingual and multilingual settings.

==> rw_last.tex <==
In this section provide a unified view of the losses used in this work (\textit{i.e} $\mathcal{L}^d_{MCMG}$, $\mathcal{L}^d_{M2CG}$, $\mathcal{L}^d_{M2CG}$ and $\mathcal{L}^u$). We follow the work from \citep{kingkong} and show that our pretraining losses can be viewed as an instance of the Infomax principle and maximize a lower bound on mutual information (MI).




Concretely we show that our newly introduce losses can be viewed as maximizing a lower
bound on the mutual information (MI) between the input context and the word composing the masked utterances. 
\subsection{Background on MI and connection to language representation learning.}
The MI is a measure of the dependence of two random variables, including high-order statistical dependencies \cite{true_mi}. Given two random variables $X$ and $Y$, the MI \cite{cover,total_correlation,multiinformation} is defined by
\begin{equation}\label{eq:mi_def}
    I(X;Y) = \mathop{\mathbb{E}_{XY}} \left[ \log \frac{p_{XY}(X,Y)}{p_X(X)p_Y(Y)} \right]
\end{equation} where $p_{XY}$ is the joint probability density function (pdf) of the random variables $(X,Y)$, and $p_X$, $p_Y$ represent the marginal pdfs. 
%MI is a measure of the difference between the joint probability $p(x,y)$ and the marginal probabilities $p(x)$ and $p(y)$, and it can be written as:
%\begin{equation}\label{eq:mi_kl}
%    I(X;Y) = H(X) - H(X | Y)
%\end{equation} where $H(X)$ represents the entropy of the r.v. X and $H(X|Y)$ represents the conditionnal entropy of $X|Y$.

In their work \citet{kingkong2} demonstrates that the masked language model objective can be linked it to InfoNCE \cite{nce,nguyen2017dual,nguyen2010estimating} which is based on Noise Contrastive Estimation \cite{gutmann2010noise}. Overall the masked language model loss can be viewed as maximising the following lower bound on MI:

\begin{align}\label{eq:mi_maximization}
    I(A,B) &\geq \mathbb{E}_{p(A,B)} [ f_\theta(a,b) - \mathbb{E}_{q(\Tilde{B})} [ \\ &\log \sum_{\Tilde{b}\in\Tilde{B}} \exp f_\theta(a,b)] + \log |\Tilde{B}|
\end{align} where in the case of masked language model b is the masked word and a is the masked sequence. Additionally, f is a scalar product \textit{i.e} $f_\theta(a,b)=g_\psi(b)^Tg_\omega(a)$ where $g_\psi$ is a look up function that map a word into a vector \textit{i.e} $g_\psi : \mathcal{V} \rightarrow \mathbb{R}^d$ and $B = \Tilde{B} = \mathcal{V}$. The proportion of the masked words can be seen as changing the joint distributions $p(a,b)$.

\subsection{Adaptation to our losses}\label{ssec:losses}
An dummy adaptation of the previous loss describes in \autoref{eq:mi_maximization} where b is the masked sentence and a is the masked context means that $|B|=|\mathbb{V}|^L$ which become intractable. Thus in our work we b is the masked token and a is the masked context. 
\\\noindent\textbf{Case of the MLM at utterance level}
\\\noindent\textbf{Case of the MLM at context level}
\\\noindent\textbf{Adaptation to the multilingual setting.}

